A Dynamic Low-Rank Fast Gaussian Transform

The \emph{Fast Gaussian Transform} (FGT) enables subquadratic-time multiplication of an $n\times n$ Gaussian kernel matrix $\mathsf{K}_{i,j}= \exp ( - \| x_i - x_j \|_2^2 ) $ with an arbitrary vector $h \in \mathbb{R}^n$, where $x_1,\dots, x_n \in \mathbb{R}^d$ are a set of \emph{fixed} source points. This kernel plays a central role in machine learning and random feature maps. Nevertheless, in most modern data analysis applications, datasets are dynamically changing (yet often have low rank), and recomputing the FGT from scratch in (kernel-based) algorithms incurs a major computational overhead ($\gtrsim n$ time for a single source update $\in \mathbb{R}^d$). These applications motivate a \emph{dynamic FGT} algorithm, which maintains a dynamic set of sources under \emph{kernel-density estimation} (KDE) queries in \emph{sublinear time} while retaining Mat-Vec multiplication accuracy and speed. Assuming the dynamic data-points $x_i$ lie in a (possibly changing) $k$-dimensional subspace ($k\leq d$), our main result is an efficient dynamic FGT algorithm, supporting the following operations in $\log^{O(k)}(n/\varepsilon)$ time: (1) Adding or deleting a source point, and (2) Estimating the ``kernel-density'' of a query point with respect to sources with $\varepsilon$ additive accuracy. The core of the algorithm is a dynamic data structure for maintaining the \emph{projected} ``interaction rank'' between source and target boxes, decoupled into finite truncation of Taylor and Hermite expansions.

==> checklist.tex <==
\section*{Checklist}




 \begin{enumerate}


 \item For all models and algorithms presented, check if you include:
 \begin{enumerate}
   \item A clear description of the mathematical setting, assumptions, algorithm, and/or model. [Yes]
   \item An analysis of the properties and complexity (time, space, sample size) of any algorithm. [Yes]
   \item (Optional) Anonymized source code, with specification of all dependencies, including external libraries. [Not Applicable]
 \end{enumerate}


 \item For any theoretical claim, check if you include:
 \begin{enumerate}
   \item Statements of the full set of assumptions of all theoretical results. [Yes]
   \item Complete proofs of all theoretical results. [Yes]
   \item Clear explanations of any assumptions. [Yes]     
 \end{enumerate}


 \item For all figures and tables that present empirical results, check if you include:
 \begin{enumerate}
   \item The code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL). [Not Applicable]
   \item All the training details (e.g., data splits, hyperparameters, how they were chosen). [Not Applicable]
         \item A clear definition of the specific measure or statistics and error bars (e.g., with respect to the random seed after running experiments multiple times). [Not Applicable]
         \item A description of the computing infrastructure used. (e.g., type of GPUs, internal cluster, or cloud provider). [Not Applicable]
 \end{enumerate}

 \item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets, check if you include:
 \begin{enumerate}
   \item Citations of the creator If your work uses existing assets. [Not Applicable]
   \item The license information of the assets, if applicable. [Not Applicable]
   \item New assets either in the supplemental material or as a URL, if applicable. [Not Applicable]
   \item Information about consent from data providers/curators. [Not Applicable]
   \item Discussion of sensible content if applicable, e.g., personally identifiable information or offensive content. [Not Applicable]
 \end{enumerate}

 \item If you used crowdsourcing or conducted research with human subjects, check if you include:
 \begin{enumerate}
   \item The full text of instructions given to participants and screenshots. [Not Applicable]
   \item Descriptions of potential participant risks, with links to Institutional Review Board (IRB) approvals if applicable. [Not Applicable]
   \item The estimated hourly wage paid to participants and the total amount spent on participant compensation. [Not Applicable]
 \end{enumerate}

 \end{enumerate}

==> discuss.tex <==
\section{Some other useful papers and techniques}



\begin{table}[h]
    \centering
    \small
    \begin{tabular}{|l|l|l|l|l|l|l|l|l|l|l|} \hline
     {\bf Refs}   & {\bf space } & {\bf  init time} & {\bf update time} &  {\bf  query time} 
       \\ \hline \hline
        CN20  & $\Tilde{O}(\epsilon^{-2}(n+d)(d+\log (1/\delta)))$ &  $\Tilde{O}(\epsilon^{-2}nd(d+\log (1/\delta)))$ &  $\Tilde{O}(\epsilon^{-2}d(d+\log (1/\delta))$  & $\Tilde{O}(\epsilon^{-2}(n+d)\log (n/\delta))$  \\ \hline
        CN22  &$O(\epsilon^{-2}nd\log(1/\delta))$  & $\Tilde{O}(\epsilon^{-2}(nd)\log (1/\delta))$ & $\Tilde{O}(\epsilon^{-2}d\log (1/\delta))$  &$\Tilde{O}(\epsilon^{-2}(n+d)\log (1/\delta))$  \\ \hline
      
    \end{tabular}
    \caption{} 
\end{table}



\begin{table}[h]
    \centering
    \begin{tabular}{|l|l|l|l|l|l|l|l|} \hline
     {\bf Refs}  
       &{\bf sketch size } & {\bf \#sketches} & {\bf subsampled \#sketches}
       \\ \hline \hline
        CN20   &$\Theta(\epsilon^{-2})$ &  $\Theta((d+\log (1/\delta)) $ & $\Theta(\log n/\delta)$  \\ \hline
        CN22  &$\Theta(d)$  & $\Tilde{\Omega}(\epsilon^{-2}\log (1/\delta))$ &   $\Tilde{\Omega}(\epsilon^{-2}\log (1/\delta))$   \\ \hline
     
    \end{tabular}
    \caption{}
\end{table}


==> sparse.tex <==


\section{Sparse Dynamic Gaussian Transform}
\begin{problem}[Dynamic heavy hitter of FGT]
Given $N$ source points $s_1,\dots,s_N \in \R^d$ with charges $q_1,\dots,q_N \in \R$ and $M $ target points $t_1,\dots,t_M \in \R^d$, find a dynamic data structure that supports the following operations:
\begin{itemize}

    \item \textsc{Insert/Delete}$(s_i,q_i )$ Insert or Delete a source point $s_i \in \R^d$ along with its ``charge'' $q_i\in \R$, in $\log^{O(d)} ( \| q \|_1 / \epsilon ) $ time. 
    
    \item\textsc{Query-Heavy-Hitter}$(\epsilon_1)$ Output the vector $v \in \R^M$ such that 
    \begin{align*}
        v_i = \begin{cases}G(t_i) \pm \epsilon, &~ \text{if } |G(t_i)| \geq \epsilon_1\\
        0,  &~ \text{otherwise}
        \end{cases}
    \end{align*}
    in $\epsilon_1^{-2} \cdot \log^{O(d)} ( \| q \|_1 / \epsilon ) $ time. 
    
    \item\textsc{Query-Set}$(S)$ Output the vector $v \in \R^M$ such that 
    \begin{align*}
        v_i = \begin{cases}G(t_i) \pm \epsilon, &~ \text{if } i \in S\\
        0,  &~ \text{otherwise}
        \end{cases}
    \end{align*}
    in $|S| \cdot \log^{O(d)} ( \| q \|_1 / \epsilon ) $ time. 
    
    \item\textsc{Query-Top}$(k)$ Output the vector $v \in \R^M$ such that 
    \begin{align*}
        v_i = \begin{cases}G(t_i) \pm \epsilon, &~ \text{if } |G(t_i)| \geq \min_{S \subset [M], |S| = k} \max_{j \notin S} |G(t_j)|\\
        0,  &~ \text{otherwise}
        \end{cases}
    \end{align*}
    in $k \cdot \log^{O(d)} ( \| q \|_1 / \epsilon ) $ time. 
\end{itemize}
\end{problem}
%

\subsection{maybe useful}
%

%

\begin{algorithm}\caption{Multiple tree}
\begin{algorithmic}[1]
\State {\bf data structure} \textsc{Multiple Tree}
\State {\bf members}
\State \hspace{4mm} $\epsilon,\delta \in (0,1)$
\State \hspace{4mm} $W \in \R^{m\times d}$ ($m $weight vectors )
\State \hspace{4mm} $X \in \R^{n \times d}$ ($n$ data points)
\State \hspace{4mm} Binary tree $T_1, T_2, \cdots, T_n$ \Comment{$n$ binary search trees}
\State \hspace{4mm} $D$ \Comment{Data Structure in Algorithm~\ref{alg:fmm_init_low_rank}}
\State {\bf end members}
\State
\Procedure{Init}{$w_1,w_2, \cdots, w_m \in \R^d, x_1, x_2, \cdots, x_n \in \R^d$} 
    \For{$i=1 \to n$}
        \State $x_i \gets x_i$
    \EndFor
    \For{$j=1 \to m$} 
        \State $w_j \gets w_j$
    \EndFor
    \For{$i=1 \to n$} \Comment{for data point, we create a tree}
        \For{$j=1 \to m$}
            \State $u_j \gets \langle x_i, w_j \rangle$ 
        \EndFor
        \State $T_i \gets \textsc{MakeBinarySearch}(u_1, \cdots, u_m)$ \Comment{Each node stores the maximum value for his two children}
    \EndFor
\EndProcedure
\State
\end{algorithmic}
\end{algorithm}

\begin{algorithm}\caption{Sparse Fast Gaussian Transform data structure}
\begin{algorithmic}[1]
\Procedure{Update}{$z\in\R^d, j \in [N]$} 
\State $s_j \gets z$ \Comment{Update source point}
\State Run FGT to obtain value of $\text{value} \gets (G q)_j$
\For{$i=1 \to n$}
    \State $l \gets$ the $l$-th leaf of tree $T_i$
    \State $l.\text{value} = \text{value}$
    \While{$l$ is not root}
        \State $p$ $\gets$ parent of $l$
        \State $p.\text{value} \gets \max \{ p.\text{value}, l.\text{value} \}$
        \State $l \gets p$
    \EndWhile
\EndFor
\EndProcedure
\end{algorithmic}
\end{algorithm}

\begin{algorithm}\caption{Multiple trees (Let $K$ denote the number entries of above $\tau$) }
\begin{algorithmic}[1]
\Procedure{Query}{$i \in [n], \tau \in \R_{\geq 0}$} \Comment{This function takes $K \cdot \log m$ time}
\State \textsc{QuerySub}($\tau,\mathrm{root}(T_i)$)
\EndProcedure
\State
\Procedure{QuerySub}{$q\in\R^d,\tau \in \R_{\geq 0}, r\in T$}
\If{$r$ is leaf}
\If{$\langle w_r,q\rangle > \tau$}
    \State \Return $r$.
\Else
    \State \Return $0$
\EndIf
\Else
\State $r_1\gets$ left child of $r$, $r_2\gets$ right child of $r$
\If{$r.\text{value} \geq \tau$}
    \State $S_1 \gets $\textsc{QuerySub}$(\tau,r_1)$
\EndIf
\If{$r.\text{value} \geq \tau$}
    \State $S_2 \gets $\textsc{QuerySub}$(\tau,r_2)$
\EndIf
\EndIf
\State \Return $S_1 \cup S_2$

\EndProcedure
\end{algorithmic}
\end{algorithm}



